Interpreting Neurons in Deep Vision Networks with Language Models

In this paper, we propose Describe-and-Dissect (DnD), a novel method to describe the roles of hidden neurons in vision networks. DnD utilizes recent advancements in multimodal deep learning to produce complex natural language descriptions, without the need for labeled training data or a predefined set of concepts to choose from. Additionally, DnD is training-free, meaning we don't train any new models and can easily leverage more capable general purpose models in the future. We have conducted extensive qualitative and quantitative analysis to show that DnD outperforms prior work by providing higher quality neuron descriptions. Specifically, our method on average provides the highest quality labels and is more than 2$\times$ as likely to be selected as the best explanation for a neuron than the best baseline. Finally, we present a use case providing critical insights into land cover prediction models for sustainability applications. Our code and data are available at https://github.com/Trustworthy-ML-Lab/Describe-and-Dissect.

==> Tables/attention_cropping_interpretability.tex <==
\begin{table}[h!]
\caption{\textbf{Effect of Attention Cropping on \algonameabbr{}.} Mean $\mu_n$ across 50 randomly chosen neurons from each layer show that attention cropping and $D_{probe}$ augmentation improve neuron interpretability by filtering out spuriously related regions in activating images.}
\label{tab:attention_cropping_interpretability}
\centering
\scalebox{0.95}{
\begin{tabular}{l|cccc}
\toprule
\multicolumn{1}{l|}{Method / Layer}  &\multicolumn{1}{c}{ Layer 1}  &\multicolumn{1}{c}{ Layer 2}  &\multicolumn{1}{c}{ Layer 3} &\multicolumn{1}{c}{ Layer 4}
\\ \hline \\
\algonameabbr{} (w/o Attention Cropping)        &0.840        &0.778         &0.729    &0.681\\
\algonameabbr{} (full pipeline)  &\bf 0.863        &\bf 0.805         &\bf 0.762    &\bf 0.712  \\ \midrule
{Improvement} &2.3\%   &2.7\%     &3.3\%     &3.1\%\\
\bottomrule
\end{tabular}
}
\end{table}

==> Tables/clip_captioning.tex <==
\begin{table}[h!]
\caption{\textbf{Mean FC Layer Similarity of CLIP Captioning.} Utilizing a fixed concept set ($\mathcal{S}$ = 20k) to caption activating images via CLIP \cite{radford2021learning}, we compute the mean cosine similarity across fully connected layers of RN50. Final labels that do not express concepts (see Figure \ref{fig:clip_captioning_failure_cases}) are given a similarity score of 0. With CLIP cosine similarity, mpnet cosine similarity, and BERTScore,  we find the performance of \algonameabbr{} w/ CLIP Captioning is slightly worse than BLIP generative caption.}
\label{tab:clip_captioning_fc}
\begin{center}
\scalebox{0.95}{
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{c|cc|c}
\toprule
\multicolumn{1}{c|}{Metric / Methods}  &\multicolumn{1}{c}{\algoname{} \textbf{(Ours)}} &\multicolumn{1}{c}{DnD w/ CLIP Captioning} &\multicolumn{1}{|c}{\% Decline}
\\ \hline
CLIP cos   &\bf0.7598   &0.7583     &0.197\%\\
mpnet cos  &\bf0.4588   &0.4465     &2.681\%\\
BERTScore  &\bf0.8286   &0.8262     &0.290\%\\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

==> Tables/concept_selection_ablation.tex <==
\begin{table*}
\caption{Human evaluation results for \algonameabbr{} (w/o Best Concept Selection) versus full \algoname{}. Full pipeline improves or maintains performance on every layer in ResNet-50.}
\label{tab:concept_selection_ablation}
\centering
\scalebox{0.95}{
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{l}{Method / Layer}  &\multicolumn{1}{c}{ Layer 1}  &\multicolumn{1}{c}{ Layer 2}  &\multicolumn{1}{c}{ Layer 3} &\multicolumn{1}{c}{ Layer 4} &\multicolumn{1}{c}{\bf All Layers}
\\ \hline \\
\algonameabbr{} (w/o Best Concept Selection)        &\bf 3.54         &3.77         &4.00     &4.02   &3.84\\
\algonameabbr{} (full pipeline)  &\bf 3.54         &\bf 4.00         &\bf 4.24     &\bf 4.13   &\bf 3.97\\
\bottomrule
\end{tabular}
}

\end{table*}

==> Tables/interpretability_exp.tex <==
\begin{table}
\caption{\textbf{Difference in Interpretability.} We compare the mean $\mu_n$ per layer for each layer in ResNet-50. Out of the original dataset from \ref{sec:scoring_fn_res}, we evaluate on the 58 neurons that were labeled as uninterpretable. }
\label{tab:interpretability_results}
\begin{center}
\scalebox{0.95}{
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{l|cccc}
\toprule
\multicolumn{1}{l|}{Classification / Layer}  &\multicolumn{1}{c}{ Layer 1} &\multicolumn{1}{c}{Layer 2}  &\multicolumn{1}{c}{Layer 3} &\multicolumn{1}{c}{Layer 4}
\\ \hline 
Interpretable  &0.863   &0.805  &0.762  &0.712\\
Uninterpretable &0.814  &0.774  &0.674  &0.655\\ \midrule
{\%Difference} &4.9\%     &3.1\%     &8.8\%     &5.7\%\\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

==> Tables/resnet-18_all_layers.tex <==
\begin{table}[!ht]
\caption{\textbf{Averaged AMT results across layers in ResNet-18}. We can see \algonameabbr{} outperforms existing methods on ResNet-18 trained on Places365. Our model was selected the best out of the three methods for more than $54\%$ of time time, almost 3$\times$ as often as the second best method.}
\label{tab:resnet18_mturk_results}
\vspace{-1em}
\begin{center}
\scalebox{0.74}{
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{c|cccc}
\toprule
% &\multicolumn{3}{c}{\bf Method}
% \\ \hline
\multicolumn{1}{c|}{Metric / Methods}  &\multicolumn{1}{c}{NetDissect} &\multicolumn{1}{c}{MILAN}  &\multicolumn{1}{c}{CLIP-Dissect} &\multicolumn{1}{c}{\algonameabbr{} \textbf{(Ours)}}
\\ \hline
Mean Rating    &3.33    &3.14    &3.52   &\bf4.14\\
selected as best  &12.62    &13.32\%     &19.39\%    &\bf54.67\%\\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

==> Tables/resnet-18_layer_ratings.tex <==
% \begin{table*}[hbt!]
% \caption{\textbf{Results for individual layers of ResNet-18}. \algonameabbr{} performs significatly better across every layer in ResNet-18 when compared to the baseline methods. Additionally, our concepts are selected over 40\% more often than any other method.}
% \label{tab:resnet18_layer_ratings}
% \begin{center}
% \scalebox{0.87}{
% \begin{tabular}{cc|ccc}
% \toprule
% &               &\multicolumn{3}{c}{\bf Method}
% \\ \midrule
% \multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c|}{\bf Layer}  &\multicolumn{1}{c}{MILAN}  &\multicolumn{1}{c}{ CLIP-Dissect} &\multicolumn{1}{c}{\thead{\algoname{} \bf(Ours)}}
% \\ \midrule
% Mean Rating         &Layer 1             &$3.20 \pm 0.119$         &$3.17 \pm 0.121$         &\bf4.07 $\pm$ \bf0.101\\
%                     &Layer 2             &$3.12 \pm 0.133$         &$3.47 \pm 0.122$         &\bf4.22 $\pm$ \bf0.086 \\
%                     &Layer 3             &$3.00 \pm 0.128$         &$3.43 \pm 0.117$         &\bf4.18 $\pm$ \bf0.081\\
%                     &Layer 4             &$3.71 \pm 0.107$         &$3.70 \pm 0.104$         &\bf4.18 $\pm$ \bf0.092\\
%  \midrule
% \% time             &Layer 1             &16.51\%         &20.18\%        &\bf63.30\% \\
% selected            &Layer 2             &16.67\%         &15.74\%        &\bf67.59\% \\
% as best             &Layer 3             &15.24\%         &20.95\%        &\bf63.81\% \\
% answer              &Layer 4             &21.49\%         &19.83\%        &\bf58.68\% \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}



% Input new results Tuomas got w/ Network Dissection
\begin{table*}[hbt!]
\caption{\textbf{Results for individual layers of ResNet-18}. \algonameabbr{} performs significantly better across every layer in ResNet-18 when compared to the baseline methods. Additionally, our concepts are selected over more than twice as often than any other method.}
\label{tab:resnet18_layer_ratings}
\begin{center}
\scalebox{0.87}{
\begin{tabular}{cc|cccc}
\toprule
&               &\multicolumn{4}{c}{\bf Method}
\\ \midrule
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c|}{\bf Layer}  &\multicolumn{1}{c}{Network Dissection}  &\multicolumn{1}{c}{MILAN}  &\multicolumn{1}{c}{ CLIP-Dissect} &\multicolumn{1}{c}{\thead{\algonameabbr{} \bf(Ours)}}
\\ \midrule
Mean Rating         &Layer 1             &$3.56 \pm 0.102$         &$3.08 \pm 0.115$         &$3.39 \pm 0.122$         &\bf4.18 $\pm$ \bf0.081\\
                    &Layer 2             &$3.03 \pm 0.107$         &$3.00 \pm 0.117$         &$3.45 \pm 0.106$         &\bf4.22 $\pm$ \bf0.082 \\
                    &Layer 3             &$3.14 \pm 0.120$         &$2.98 \pm 0.114$         &$3.46 \pm 0.108$         &\bf4.08 $\pm$ \bf0.079\\
                    &Layer 4             &$3.60 \pm 0.110$         &$3.49 \pm 0.116$         &$3.77 \pm 0.100$         &\bf4.10 $\pm$ \bf0.081\\
 \midrule
\% time             &Layer 1             &15.09\%         &11.32\%         &19.81\%        &\bf53.77\% \\
selected            &Layer 2             &6.31\%         &11.71\%         &19.82\%        &\bf62.16\% \\
as best             &Layer 3             &14.29\%         &12.38\%         &15.24\%        &\bf58.10\% \\
answer              &Layer 4             &15.09\%         &17.92\%         &22.64\%        &\bf44.34\% \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

==> Tables/resnet-50_all_layers.tex <==
\begin{table}[!ht]
% \caption{\textbf{Averaged AMT results across layers in ResNet-50}. We can see our descriptions are consistently rated the highest, rated between \textit{Agree} and \textit{Strongly Agree}. Our method is also chosen as the best description $>50\%$ of the time, more than twice as often as the best baseline. The std of rating is small (0.022 to 0.032).}
\caption{\textbf{Averaged AMT results across layers in ResNet-50}. Our descriptions are consistently rated the highest and chosen as the best more than twice as often as the best baseline.}
\label{tab:resnet50_mturk_results}
% \vspace{-1em}
\begin{center}
\scalebox{0.75}{
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{c|cccc}
\toprule
% &\multicolumn{4}{c}{\bf Method}
% \\ \hline
\multicolumn{1}{c|}{Metric / Method}  &\multicolumn{1}{c}{NetDissect}  &\multicolumn{1}{c}{MILAN}  &\multicolumn{1}{c}{CLIP-Dissect} &\multicolumn{1}{c}{\thead{\algonameabbr{} \bf(Ours)}}
\\ \hline 
Mean Rating    &3.14 $\pm{0.032}$        &3.21 $\pm{0.032}$         &3.67 $\pm{0.028}$       &\bf4.15 $\pm{0.022}$ \\
Selected as Best   &12.71\%         &13.29\%         &23.11\%        &\bf50.89\% \\
\bottomrule
\end{tabular}

}
\end{center}
\vspace{-1em}
\end{table}

==> Tables/resnet-50_layer_ratings.tex <==
\begin{table*}
\caption{\textbf{Results for individual layers of ResNet-50}. We observe that \algonameabbr{} is the best method across all layers in ResNet-50. Our concepts achieved a mean rating of over 4.0 for every layer and were 2$\times$ as likely to be selected as the best concept when compared to baseline methods.}
\label{tab:resnet50_layer_ratings}
\begin{center}
\scalebox{0.87}{
\begin{tabular}{cc|cccc}
\toprule
&               &\multicolumn{4}{c}{\bf Method}
\\ \midrule
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c|}{\bf Layer}  &\multicolumn{1}{c}{Network Dissection} &\multicolumn{1}{c}{MILAN}  &\multicolumn{1}{c}{CLIP-Dissect } &\multicolumn{1}{c}{\algonameabbr{} \bf(Ours)}
\\ \midrule 
Mean Rating          &Layer 1             &$3.41 \pm 0.058$         &$3.41 \pm 0.060$         &$3.63 \pm 0.057$         &\bf4.16 $\pm$ \bf0.041 \\
                    &Layer 2             &$3.14 \pm 0.067$         &$3.12 \pm 0.064$         &$3.55 \pm 0.057$         &\bf4.07 $\pm$ \bf0.048 \\
                    &Layer 3             &$3.04 \pm 0.066$         &$2.96 \pm 0.066$         &$3.66 \pm 0.055$         &\bf4.14 $\pm$ \bf0.042 \\
                    &Layer 4             &$2.97 \pm 0.066$         &$3.34 \pm 0.061$         &$3.82 \pm 0.054$         &\bf4.21 $\pm$ \bf0.044 \\  \midrule
\% time             &Layer 1             &13.18\%         &14.32\%         &22.50\%         &\bf50.00\% \\
selected            &Layer 2             &15.27\%         &12.41\%         &19.33\%         &\bf52.98\% \\
as best             &Layer 3             &11.82\%         &12.73\%         &25.00\%         &\bf50.45\% \\
answer              &Layer 4             &10.56\%         &13.71\%         &25.62\%         &\bf50.11\% \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}
